Improving AoI via Learning-based Distributed MAC in Wireless Networks

In this work, we consider a remote monitoring scenario in which multiple sensors share a wireless channel to deliver their status updates to a process monitor via an access point (AP). Moreover, we consider that the sensors randomly arrive and depart from the network as they become active and inactive. The goal of the sensors is to devise a medium access strategy to collectively minimize the long-term mean network \ac{AoI} of their respective processes at the remote monitor. For this purpose, we propose specific modifications to ALOHA-QT algorithm, a distributed medium access algorithm that employs a policy tree (PT) and reinforcement learning (RL) to achieve high throughput. We provide the upper bound on the mean network Age of Information (AoI) for the proposed algorithm along with pointers for selecting its key parameter. The results reveal that the proposed algorithm reduces mean network \ac{AoI} by more than 50 percent for state of the art stationary randomized policies while successfully adjusting to a changing number of active users in the network. The algorithm needs less memory and computation than ALOHA-QT while performing better in terms of AoI.

==> Images/fully_unbalanced_5.tex <==
\tikzset{every tree node/.style={minimum width=1.5em,draw,circle},
         blank/.style={draw=none},
         edge from parent/.style=
         {draw,edge from parent path={(\tikzparentnode) -- (\tikzchildnode)}},
         level distance=1.4cm, level 1/.style={sibling distance=2mm},level 2/.style={sibling distance=2mm}, level 3/.style={sibling distance=5mm}}
\begin{tikzpicture}
\Tree
[.\node[label={(0,0)}]{}; 
    [. \node[label={(0,2)}, fill=FillColor0!60]{};
    ]
    [.\node[label={{(1,2)}}]{};
    [. \node[label={(1,4)}, fill=FillColor0!60]{};
    ]
    [.\node[label={(3,4)}]{};
    [.\node[label={(3,8)}, fill=FillColor0!60]{};
    ]
    [.\node[label={(7,8)}]{};
    \node[label={(7,16)}, fill=FillColor0!60]{};
    \node[label={(15,16)}, fill=FillColor0!60]{};
    ]
    ]
    ]
]
\end{tikzpicture}

